Adaptive whitening with fast gain modulation and slow synaptic plasticity

Neurons in early sensory areas rapidly adapt to changing sensory statistics, both by normalizing the variance of their individual responses and by reducing correlations between their responses. Together, these transformations may be viewed as an adaptive form of statistical whitening. Existing mechanistic models of adaptive whitening exclusively use either synaptic plasticity or gain modulation as the biological substrate for adaptation; however, on their own, each of these models has significant limitations. In this work, we unify these approaches in a normative multi-timescale mechanistic model that adaptively whitens its responses with complementary computational roles for synaptic plasticity and gain modulation. Gains are modified on a fast timescale to adapt to the current statistical context, whereas synapses are modified on a slow timescale to match structural properties of the input statistics that are invariant across contexts. Our model is derived from a novel multi-timescale whitening objective that factorizes the inverse whitening matrix into basis vectors, which correspond to synaptic weights, and a diagonal matrix, which corresponds to neuronal gains. We test our model on synthetic and natural datasets and find that the synapses learn optimal configurations over long timescales that enable adaptive whitening on short timescales using gain modulation.

==> rebuttals.tex <==
\newcommand{\lyndon}[1]{{\color{RoyalBlue}LD: #1}}
\newcommand{\eero}[1]{{\color{ForestGreen}EPS: #1}}
\newcommand{\mitya}[1]{{\color{Fuchsia} MBC: #1}}
\newcommand{\rebuttal}[1]{{\color{Plum} #1}}
\newcommand{\david}[1]{{\color{RubineRed}DL: #1}}

\section{Rebuttals}

\subsection{General response}

\david{
We thank the reviewers for their careful reading of our work and for their helpful comments. We have revised our paper in accordance with your suggestions and provide individual responses to your comments. Here we list general changes and additions to the manuscript.

1. We tested Algorithm 3, the more biologically realistic multi-timescale version of our online algorithm, on a synthetic dataset and found that it successfully learned optimal filters and was able to adaptively whiten the data using gain modulation, Figure E.2 of the attached PDF.

2. We tested the effect of varying the $\alpha$ parameter on the synthetic dataset, Figure E.3 of the attached PDF. We find that when the column vectors of ${\bf V}$ are orthogonal, varying $\alpha$ does not affect the performance of the algorithm; however, when ${\bf V}$ are not orthogonal, there is a slight degradation of performance when $\alpha$ is not exactly 1. This is due to the fact that if ${\bf V}$ is orthogonal (and full rank), then $\alpha{\bf I}+{\bf V}\Lambda {\bf V}^\top$ can be decomposed as ${\bf V}(\alpha{\bf I}+\Lambda){\bf V}^\top$, so the basis vectors for the (inverse) whitening matrix do not depend on $\alpha$.

3. We propose changing the title from ``Multiscale adaptive whitening in neural circuits with synaptic plasticity and gain modulation'' to ``Adaptive whitening with slow synaptic plasticity and rapid gain modulation'' to more effectively convey the central computation of the model.

}

\subsection{Reviewer 1 yTCH: 6(3)}

\subsubsection*{Weaknesses}
I don't have major concerns about this study from the math point of view. Nonetheless, I have a significant concern from the neuroscience point of view.

The derived updating rule of gain (Eq. after line 174) depends on the current weight. The neural "gain" is typically adjusted by inhibitory interneurons, and thus I am concerned about how interneurons "sense" the synaptic weights. If there are neurobiological studies supporting this updating rule, please cite the reference in the paper, otherwise, it is better to discuss it at the end.

% \lyndon{Thanks for voicing this concern. Although it's not so apparent in the main text,  we've resolved this issue in Appdx D.1 . Specifically, we scale the synaptic weights to have have constant norm. This effectively replaces the $\text{diag}(W^\top W)$ term with a constant. This is reminiscient of the synaptic scaling/synaptic redistribution mechanisms proposed by Abbott + Nelson (2000). 
% Additionally, if the timescale of weight updates, $\eta_w$, is sufficiently slow, and weights are near-optimal across contexts (i.e. $\mathbb{E}_{c\sim p(c)}[C_{ss}(c)]$), then the target term is effectively constant. 
% }

% \david{We can appeal to a weight normalization mechanism that scales the synaptic weights so that have constant norm (e.g. Appendix Eq. D.1). In this case, we can replace the $\text{diag}({\bf W}^\top{\bf W})$ term with $\vone$.}

% \david{We can point to synaptic scaling or synaptic redistribution \citep{abbott2000synaptic} as mechanisms that approximately normalize $\text{diag}({\bf W}^\top{\bf W})$. They are slightly different formulations, but the general proposed mechanisms could be useful.}

\subsubsection*{Questions}
\begin{enumerate}
    \item  Line 91: ref. 11 requires $K\geq N$
, i.e., the number of I neurons is larger than the E neurons. Does this requirement also need in this paper? Is there a way to make the number of I neurons less than the E neurons? This is also the case in the cortex.
\item It seems that the $f_c(M)$
 function was used before but the writing still looks abrupt to me about why to propose an objective function with such a form.
\item The paragraph starting at line 90. It is better to first explain the decomposition $M_C=W_CW_C^\top$
 regards to the weights between E and I neurons. Otherwise, people can easily regard  as the feedforward weights.
\end{enumerate}
% \lyndon{Q1: 
% Yes, for cases such as in the cortex when $K<N$, it's still possible to produce whitened responses.  This occurs when the (inverse) whitening matrix lies on a low-dimensional subspace. Further, some experiments in cortex (Benucci et al. 2013) have shown that primary neurons reduce redundancy after adaptation, but are not perfectly whitened -- $K<N$ may provide an explanation for this effect.

% Q2+3: Thanks for pointing this out, we will amend the text as you suggest to improve clarity.}

 \subsubsection*{Limitations}
I realize the framework assumes the synaptic weights between excitatory (E) and inhibitory (I) neurons are symmetric with each other by just differing a sign. Is there a way to break this symmetry? Will the symmetry breaking of E-I weights facilitate optimization?

% \lyndon{ We discuss weight decoupling in Appendix D.2. We'd also like to mention that reciprocal connections between excitatory and inhibitory neurons have been observed in structures such as the olfactory bulb (Shepard 2004; Friedrich 2013), where dendrodendritic synapses give rise to symmetric connectivity matrices (although, not necessarily symmetric weight matrices). An exploration of circuit function with asymmetric weights (e.g. for non-symmetric whitening transforms) is an interesting future direction to pursue.
% }

\rebuttal{

Thank you for your review and thoughtful questions.

Weaknesses:

Thanks for voicing this concern. Although it's not so apparent in the main text,  we've resolved this issue in Appdx D.1 . Specifically, we scale the column vectors of ${\bf W}$ to have have constant norm 1. This effectively replaces the $\text{diag}(W^\top W)$ term with a constant vector of ones, so gain updates do not need to ``sense'' the synaptic weights. This is reminiscent of the synaptic scaling/synaptic redistribution mechanisms discussed in Abbott \& Nelson (2000). 
Additionally, when the weights are near-optimal, then they are approximately constant across contexts and the target term is effectively constant. 

Questions: 

1. Yes, for cases such as in the cortex when $K<N$, it's still possible to produce whitened responses provided the set of (inverse) whitening matrices lie within a $K$-dimensional subspace. Further, some experiments in cortex (Benucci et al. 2013) have shown that primary neurons reduce redundancy after adaptation, but are not perfectly whitened; $K<N$ may provide an explanation for this effect.

2. Thanks for pointing this out, we will amend the text as you suggest to improve clarity.

3. Thanks, we will make this change in conjunction with the previous one.


Limitations:

We discuss weight decoupling in Appendix D.2. But it is worth mentioning that reciprocal connections between excitatory and inhibitory neurons have been observed in structures such as the olfactory bulb (Shepard 2004; Friedrich 2013), where dendrodendritic synapses give rise to symmetric connectivity matrices (although, not necessarily symmetric weight matrices). An exploration of circuit function with asymmetric weights (e.g. for non-symmetric whitening transforms) is an interesting direction to pursue. Preliminary findings suggest that non-symmetric weights can lead to non-symmetric whitening transformations.
}


% \david{I would point to Appendix D.2 where we decouple the weights. Not just the zebrafish olfactory bulb, but also the mammalian olfactory bulb (Shepard 2004). We can explicitly mention the dendrodendritic synapses, which implies symmetric connectivity matrices (though not necessarily symmetric weight matrices).}

\subsection{Reviewer 2 3ayL: 7(5)}

\subsubsection*{Weaknesses}
There are no significant weaknesses in this paper. To the authors’ credit, every question I had that I thought was in the category of “necessary for publication” they addressed. I’ll leave everything else to “Questions”, below.

The biggest weakness I see regards the generality of the matrix decomposition. The extent to which the authors test or address this appears on par with other approaches in the field, though. I have some questions below on this topic.

\subsubsection*{Questions}
\begin{enumerate}
\item  Can you make any statements about how general the matrix decomposition in Section 3.3 is? It seems very specific. You demonstrate numerically that this decomposition works for your experiment. When do you expect it to fail? Can you characterize or quantify the differences in context necessary before this decomposition no longer works? 

% \david{We can be precise in describing the set of covariance matrices that can be whitened with this decomposition. In particular, when the (inverse) whitening matrices lie in a low-dimensional subspace, this is an efficient representation. It appears to be efficient for natural image statistics which approximate share eigenvectors. I'd expect it to be less efficient when the (inverse) whitening matrices do not lie in a low-dimensional subspace, but perhaps this can explain why some circuits have an abundance of interneurons (e.g., olfactory bulb).}

\item Related to this, it looks like you’re using images from the van Hateren database. Can you try the held out image experiments with images from very different contexts and origins, since those images all have clear similarities in large scale properties? This might help find the limits of this algorithm/decomposition.

% \lyndon{This is an interesting question which can be answered by appealing to well-known results from image/video coding literature: a sinusoidal basis (e.g. the DCT) approximates the Karhunen Loeve Transform, an optimal basis for natural images (Ahmed 1974; Bull and Zhang 2021). Our algorithm learns an approximately orthogonal sinusoidal basis as interneuron weights $W$ without supervision (Fig 4D, 4F, C.1B, C.2); therefore, this trained model is well-suited to held-out test images whose statistics do not deviate too far from those of natural images.}

\item I was going to ask about breaking the symmetry on the weights, which you answered in an appendix. They will asymptotically align, but can you say something about this timescale? Is there a restriction on when the alignment has to happen with respect to the gain modulation and synaptic plasticity that is meaningful or prohibitive?

% \david{I'd point to Appendix D.2 for decoupling the weights. Also, olfactory bulb.}

% \lyndon{they already mention appdx discussion. can u answer this one since i think they're asking how fast this weight-symmetry convergence happens wrt gain and plasticity timescales. }

% \david{Yes. As shown in Appendix D.2, the convergence to symmetric weights is exponential. If the weights are order 1, then the exponential convergence rate is on the order $-\log(1-\eta_w)\approx\eta_w$ when $\eta_w$ is small. Therefore, the convergence rate is exponential with convergence rate determined by the learning rate for the synaptic weight updates.}

\item You provide the error as a function of number of interneurons for your natural image experiment. Can you compute some normalization so that there is an idea of what errors are meaningful (maybe the Frobenius norm of C)? 

\item Your interneurons are not necessarily the “interneurons” people talk about in real circuits, but it makes one imagine nonetheless that you will have far fewer interneurons than primary neurons. Is this a functional problem given the amount of error you see? Maybe it’s “good enough” even with few interneurons?


% \lyndon{
% First, we'd like to point out that this proportion of interneurons is in fact a relevant scenario in the olfactory bulb, where interneurons outnumber excitatory neurons by up to 100:1 (Shepard 2004; Friedrich 2013). 
% Second, we show in Fig 4E and Appendix C shows that our network transitions gracefully to the regime where $K\ll N$. (e.g. in neocortex it is roughly 1:3)
% }

\david{We can point to Fig 4E to show that error is reasonable even when there are fewer interneurons. Maybe it would look better if we use Frobenius norm? Since neocortex is 1:3, a possibility would be to show the spectrum of the response covariance matrix (not error) when $K=5$ (vs.\ when $K=0$) in the example shown in Figure C.2.}
\end{enumerate}

 \subsubsection*{Limitations}
The authors do not discuss societal impact.

\rebuttal{
We appreciate your positive review and thoughtful questions about the work!

Questions:

1. We can be precise in describing the set of covariance matrices that can be whitened with this decomposition. In particular, when the inverse whitening matrices lie in a $K$-dimensional linear subspace, then this representation can match the whitening matrices with $K$ interneurons. Since the covariance matrices of natural images approximately share an eigen-basis, this representation can approximately match the corresponding whitening matrices with $K=N$. When the inverse whitening matrices do not lie in a low-dimensional linear subspace, we expect that the representation will require $K$ to be much larger, which can perhaps explain why some circuits have many more interneurons than primary neurons (e.g., olfactory bulb).

2. This is an interesting question which can be answered by appealing to well-known results from the image/video coding literature: a sinusoidal basis (e.g. the DCT) approximates the Principal components (Karhunen Loeve Transform) for natural images (Ahmed 1974; Bull and Zhang 2021). Our algorithm learns an approximately orthogonal sinusoidal basis as interneuron weights ${\bf W}$ without supervision (Fig 4D, 4F, C.1B, C.2); therefore, this trained model is well-suited to any held-out test images (e.g., outside the van Hateren database) whose statistics do not deviate too far from those of natural images.

3. Yes, as we show in Appendix D.2 that the convergence to symmetric weights is exponential. If the weights are order 1, then the exponential convergence rate is on the order $-\log(1-\eta_w)\approx\eta_w$ when $\eta_w$ is small. That is, the convergence rate is determined by the learning rate for the synaptic weight updates.

4. Thanks for pointing out this issue of interpretability of the error plots. To provide a better sense of error improvement, we've added a horizontal reference line to show what the error would be with no interneurons (i.e. without whitening).

5.  For olfactory bulb, it seems that this proportion of interneurons is in fact a relevant scenario: interneurons can outnumber excitatory neurons by up to 100:1 (Shepard 2004; Friedrich 2013). 
We do show in Fig 4E and Appendix C that our network transitions gradually to the regime where $K\ll N$. In this regime when $K<N$, the error is indeed significantly improved (relative to no whitening --- horizontal line in PDF Fig E.1).
}

\subsection{Reviewer 3 NSc1: 7(4)}

\subsubsection*{Weaknesses}

Some weaknesses are inherited from the Duong et al.~[18] model which this paper is building on, specifically related to its biological plausibility:
\begin{enumerate}
    \item All neurons are linear.

    \item Dale's law is not observed.

    \item Forward and backward weights are mirrored.

    \item In general, more interneurons than excitatory neurons are required (in the worst case, as many as $O(n^2)$
 interneurons for $n$
 excitatory neurons), which does not match the ratios observed in the brain. Experimentally, the algorithm fails gracefully when fewer interneurons than required are available. A more realistic version of the model which addresses the first two issues is provided in the appendix. However, given that the scope of this work is primarily modeling a phenomenon in neuroscience, I think the paper would be stronger if this biologically plausible version were featured and evaluated more prominently.

 % \lyndon{Weakness 1-3 are all valid comments and are indeed inherited from existing frameworks upon which our model is built. Point 1: by adding nonlinearity is an interesting idea for an extension worth pursuing in a future study. We will update an included reference on related work by Chapochnikov et al. (2023) containing analyses on rectifying interneuron responses. Point 2: has been addressed in e.g. Algo 3 in the Appendix which allows the network to abide by Dale's law. Point 3: a discussion on weight symmetry is included in Appendix D.}

 % \david{For point 1, we can also point to Chapochnikov et al.\ 2023 for analysis about what happens when the interneurons are rectified.}
 
 % \lyndon{Point 4: First, interneurons outnumbering excitatory neurons is in fact a relevant phenomenon observed in neuroscience, and exists in structures such as the olfactory bulb, where interneurons outnumber primary neurons by up to 100:1 (Friedrich, 2013).}
\end{enumerate}


\subsubsection*{Questions}

\begin{enumerate}
\item Line 83: Missing a trace on the RHS of the equation?

% \lyndon{Thanks for pointing this out. We have corrected this equation.}

\item I would appreciate a more in-depth evaluation, perhaps on a synthetic dataset, of what happens when there are fewer interneurons than required.

% \lyndon{Refer to Fig 4E (natural images example), and Appendix C.
% Because of the L2 reconstruction error, (approximately) progressively learns eigenvectors of the average covariance across all contexts $\mathbb{E}_{c \sim p(c)}[C_{ss}(c)]$.
% We have now also included the case with no interneurons ($K=0$) and therefore no whitening, for 
% }

% \david{Also point to Fig 4E. Can we include the case of zero interneurons?}

% \lyndon{will do.}

\item Did you consider adding an activation function, at least to the interneurons? I could imagine that there is a similar learning algorithm which allows for fewer nonlinear interneurons.

% \lyndon{This is great suggestion for an extension to the model! Adding a nonlinear activation to the interneuron activations may indeed allow for a smaller number of interneurons $K$. Recent related work by Chapochnikov et al. (2023) analyze the use rectified interneurons in the context of similarity-matching-based olfactory circuit adaptation. 
% Here, we were focused on introducing the novel concept of multi-timescale whitening, and wish to keep the computation as analytically tractable as possible with this added layer of complexity. Any definitive claims on the whitening capability of our network with nonlinearities warrants a separate, follow-up study with extensive numerical/empirical investigation.
% }

% \david{Point to Chapochnikov et al.\ 2023 for analysis about what happens when the interneurons are rectified. To reiterate your point, we can say this study is focused on multi-timescale whitening and we want to keep things as analytically tractable as possible while adding this extra layer of complexity.}
\end{enumerate}


\subsubsection*{Limitations}
% Yes.

% \hl{Still need to finish Weakness4 and Q2}

% \rebuttal{

% Weaknesses:

% We agree these are weaknesses (perhaps, "simplifications", "approximations"), but all are inherited from existing frameworks upon which our model is built, and most are addressed in the paper:

% 1. We agree that incorporating nonlinearity is an important extension worth pursuing in a future study. We will add to related work a paper by Chapochnikov et al. (2023) containing analyses on rectifying interneuron responses. 

% 2. Algo 3 in the Appendix allows the network to abide by Dale's law. 

% 3. A discussion of weight symmetry is included in Appendix D.

% 4. Ratios of interneurons to excitatory neurons varies in neural systems. In the olfactory bulb, interneurons outnumber primary neurons by up to 100:1 (Friedrich, 2013).

% Questions: 

% 1. Thanks for pointing this out. We have corrected this equation.

% 2. Refer to Fig 4E (natural images example), and Appendix C.
% Because of the L2 reconstruction error, (approximately) progressively learns eigenvectors of the average covariance across all contexts $\mathbb{E}_{c \sim p(c)}[C_{ss}(c)]$.
% We have now also included the case with no interneurons ($K=0$) and therefore no whitening.

% 3. This is great suggestion for an extension to the model! Adding a nonlinear activation to the interneuron activations may indeed allow for a smaller number of interneurons $K$. Recent related work by Chapochnikov et al. (2023) analyzes the role of rectifying interneurons in the whitening olfactory circuit in the context of similarity-matching-based adaptation. 
% Here, we were focused on introducing the novel concept of multi-timescale whitening, and wish to keep the computation as analytically tractable as possible with this added layer of complexity. Any definitive claims on the whitening capability of our network with nonlinearities warrants a separate, follow-up study with extensive numerical/empirical investigation.

% }

\david{
Thank you for your careful review and for your useful comments. We appreciate your comment that our model has broader implications for ML and applications to transfer learning.

Weaknesses: We readily acknowledge there are aspects of our model that are not biologically realistic. This is in part due to the fact that the model is derived from an objective that can whiten any input distribution, which is perhaps unrealistic for a biological system. While we did not have space to fully address this in the main paper, in Algorithm 3 of Appendix D, we considered modifications of our circuit to improve its biological realism. 

1. By adding nonlinearity is an interesting idea for an extension worth pursuing in a future study. We will update an included reference on related work by Chapochnikov et al. (2023) containing analyses on rectifying interneuron responses. 

2. In Appendix D.2 we decouple the feedforward and feedback weight updates and in Appendix D.3 we consider a modified synaptic update rule that enforces Dale's law. In Figure E.2 of the attached PDF, we show that the modified algorithm indeed works on synthetic datasets.

3. See Weakness 2. above.

4. First, interneurons outnumbering excitatory neurons is in fact a relevant phenomenon observed in neuroscience, and exists in structures such as the olfactory bulb, where interneurons outnumber primary neurons by up to 100:1 (Friedrich, 2013). Second, in Figure E.1 of the attached PDF, we show that even when $K\ll N$, the circuit responses which be much more decorrelated than the circuit inputs. This approximate decorrelation using fewer interneurons can perhaps explain why responses in V1 are only close to decorrelated (Benucci et al., 2013).

Questions: 

1. Thanks for pointing this out. We have corrected this equation.

2. In Fig 4E (natural images example) and Appendix C, we carefully analyze the effect of having fewer interneurons than required. In Fig 4D, we show that the ``whitening error'' gradually decreases with the number of interneurons $K$ until $K=N$, at which point there is a discontinuous decrease that is due to the fact that we are measuring the difference using the operator norm. We see that even for $K\approx N/3$, which corresponds to the ratio of interneurons to primary neurons in the cortex, the whitening error is much smaller than when $K=1$.
We have now also included the case with no interneurons ($K=0$) and therefore no whitening, see Figure E.1 of the attached pdf.

3. This is great suggestion for an extension to the model! Adding a nonlinear activation to the interneuron activations may indeed allow for a smaller number of interneurons $K$. Recent related work by Chapochnikov et al. (2023) analyzes the role of rectifying interneurons in the whitening olfactory circuit in the context of similarity-matching-based adaptation. 
Here, we were focused on introducing the novel concept of multi-timescale whitening, and wish to keep the computation as analytically tractable as possible with this added layer of complexity. Any definitive claims on the whitening capability of our network with nonlinearities warrants a separate, follow-up study with extensive numerical/empirical investigation.

}


\subsection{Reviewer 4 yS92: 5(4)}

% \lyndon{Dear Reviewer yS92, thank you for your thoughtful review. We have addressed all your comments below, but are concerned you may be focusing on points which are not central contributions of our work. We emphasize that our study's primary motivation is not simply about whitening, but to develop a biologically realistic circuit for \textit{context-dependent} whitening, which is subtly distinct from prior work. We formalize existing mechanisms of gain modulation and synaptic plasticity into a joint computation conducted across multiple timescales, thereby yielding a new mechanistic theory and sensible solution to context-dependent adaptation in neural circuits. As we understand, this type of approach has not yet been done, and its novelty and importance should not be discounted.
% }

% \david{Quotes from other reviewers: \\ \\
% Reviewer yTCH: ``The strength of this paper is that it combines the fast gain modulation and slow synaptic plasticity in a whitening neural circuit, and addresses the shortcomings of earlier models with either gain modulation or synaptic plasticity.'' \\ \\
% Reviewer 3ayL: ``This is a very nice paper that connects the computational problem of whitening with multiple neural mechanisms into a single normative framework''
% }

\subsubsection*{Weaknesses}
The writing is lacking in some parts, and some important details are missing in the paper. More numerical experiments should be presented to assess the introduced framework. For exact details on the weaknesses, please see my comments below and questions section.

% \david{Thank you for your careful reading of our work and for your suggestions. We regret that you found the writing lacking in some parts. We believe that the weaknesses you point out are important, but can be readily addressed. We have carefully edited the paper according to your suggestions, which we believe has improved the overall clarity of our work.}

\begin{enumerate}
    \item Line 83, "... where $f_c(M_C)=2M_C$
" should be changed to "... where $f_C(M_C)=Tr(2M_C)$
" since $f_c$
 is a scalar function of matrices. Moreover, even though it is a simple proof, it would be valuable how this unique minimum is achieved.
 
 % \lyndon{Thanks, we have corrected this equation.}
 
 \item 
The intermediate step (stated between line 150 and line 153) to obtain Equation (4) should be written explicitly in the paper (can be in the appendix).

% \lyndon{We will add a short section to the appendix with the intermediate steps laid out.}

\item 
The decoupling the feedforward and feedback weights (in Appendix D.2) is very similar to the idea presented in [i] since the assumption $g_i+m_i \in (0, 2 \eta^{-1}_w$ corresponds to weight decaying. The paper should cite this reference. 
[i]J.F. Kolen and J.B. Pollack. Backpropagation without weight transport. In Proceedings of 1994 IEEE International Conference on Neural Networks (ICNN’94), volume 3, pages 1375–1380 vol.3, 1994. doi: 10.1109/ICNN.1994.374486.

% \lyndon{Thanks, we will include this reference in the text of this section.}

\item For the experiment with synthetic data, the experiment only considers the whitening matrix of the form $M_c = I_N + V\Lambda(c) V^\top$
. An experiment with more general form of whitening matrix is required to assess the performance of the proposed algorithm.

% \david{A strength of our normative approach to deriving a neural circuit is that its performance can be predicted by analyzing the starting objective. In particular, given W, we can analytically describe the set of covariance matrices that can be whitened by the circuit (see the display after eq 3). Our numerical simulations verify this analytical prediction. Therefore, while we think that further experiments would further validate our analytical predictions, we believe that given the analytical nature of our results, the current set of experiments adequately validates the performance of the circuit.}

\item Hyperparameters (i.e., $\eta_w, \eta_g. \eta_r$
) are not provided in the paper (except that the authors provide 
 for Algorithm 2 in Appendix C). It would be beneficial for the paper to include a table that provides the hyperparameters used in each experiment

% \lyndon{Thanks for pointing this out. We will amend the text to include a table of these hyperparameters.}

\item The differences and novelties compared to previous works by Pehlevan and Chklovskii [11] and Duong et al. [18] are discussed quite well, but the comparison in the numerical experiments is missing.

% \lyndon{The Pehlevan and Chklovskii vs Duong et al. models correspond to our network when $\eta_g=0$ and $\eta_w=0$, respectively.
% These regimes are examined in the natural image dataset in Fig. 4C.
% We will amend the text to more clearly emphasize and explain this.
% }

% perhaps add more..? idk

\item A single Python script is shared for the proposed method, although it does not include the experiment code. The authors mentioned in the paper that the full code would be shared upon publication. However, the current code does not provide a comprehensive understanding of the conducted experiments.

% \lyndon{Thanks for your interest in seeing more detail.  We provide self-contained code to better understand the conducted experiments (anonymous link submitted to the AC, as instructed).}

\end{enumerate}

\subsubsection*{Questions}
\begin{enumerate}
    \item The numerical experiments presented in Appendix C uses Algorithm 2, but the biological plausibility of it is questionable due to matrix inversion and batch learning. Did you experiment with this setup using Algorithm 1?
    
    % \lyndon{We did this experiment with Algorithm 1; see the rebuttal pdf figure XXX. As you can see, it does not change the qualitative end-result; the main difference is that it requires more iterations.}
    
    \item  The authors propose Algorithm 3 as more biologically plausible algorithm compared to the Algorithm 1, by complying to the Dale's law and decoupling the feedforward and feedback weights for asymmetry (weight transport problem). However, no numerical experiment has been demonstrated for this proposal. Did you test this algorithm?
    
    \item The value of $\alpha$ seems to be also an hyperparameter for the proposed framework. Did you analyze the effect of this choice?
\end{enumerate}


\subsubsection*{Limitations}
I think that the limitations are adequately discussed in the paper.

\david{
Thank you for your careful reading of our work and for your suggestions. We regret that you found the writing lacking in some parts. We have revised our paper in accordance with your suggestions (see our detailed responses below), which we believe has improved the overall clarity of the paper.

We are concerned that a central contribution of our work may not have been appreciated. Our primary motivation is to develop a biologically realistic circuit for adaptive, \textit{context-dependent} whitening with complementary computational roles for synaptic plasticity and gain modulation. We formalize existing mechanisms of gain modulation and synaptic plasticity into a joint computation operating across multiple timescales, yielding a new mechanistic theory and solution to context-dependent adaptation in neural circuits. We believe this is a novel and significant contribution, which we will emphasize in our revision.

Weaknesses:

1. We corrected the equation and added a short proof that explains how the minimum is achieved.

2. We added a short section to the appendix with the intermediate steps written explicitly.

3. Thank you for pointing us to reference [i]. It is indeed relevant and we've added a citation.

4. A strength of our normative approach is that its performance can be predicted by analyzing the starting objective. In particular, given ${\bf W}$, we can analytically describe the set of covariance matrices that can be whitened by the circuit (see the display after eq 3). Our numerical simulations verify this analytical prediction. Given the analytical nature of our results, we believe that the current set of experiments adequately validates the performance of the circuit.

5. We amended the text to include a table of these hyperparameters.

6. The Pehlevan and Chklovskii [11] and Duong et al.~[18] models, which respectively use either synaptic plasticity or gain modulation, correspond to our network in the regimes $\eta_g=0$ and $\eta_w=0$, respectively. A comparison of these regimes is shown in Fig.~4C, where we quantify the test error for our model (red histogram), for fixed gains [11] (green histogram) and for fixed synapses [18] (purple histogram). We amended the text to emphasize this comparison to previous work.

7. We have submitted full code (to the AC via an anonymous link, as instructed) for the synthetic data experiments.

Questions:

1. Yes, using the Algorithm 1 for e.g. Appendix Fig C.1 still learns an approximately orthogonal sinusoidal basis for the data. The main difference is that the online algorithm requires far more iterations than the offline algorithm.

2. Yes, see Fig E.2 in the rebuttal PDF. 

3. Yes, we've analyzed the $\alpha$ parameter, which corresponds to the leak term in the neural dynamics. In the context of the synthetic experiment when the generative basis, $V$, is not orthogonal, a non-zero $\alpha$ parameter is necessary (effectively due to the matrix inversion); when $V$ is orthogonal, $\alpha$ is less important and can be set to zero. See Fig E.3 in rebuttal PDF.
}

\newpage
\thispagestyle{empty}

% \begin{figure}
%     \centering
%     \includegraphics[width=.4\textwidth]{figures/rebuttal_k0.png}
%     \caption{Same as Fig.~4E, but with error when $K=0$ (i.e. without whitening) plotted as horizontal reference line. Notably, even in the $K<N$ regime, error is substantially improved relative to $K=0$.}
%     \label{fig:k=0}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=.7\textwidth]{figures/rebuttal_algo3b.png}
%     \caption{With stricter constraints on biological realism (Appendix D.4; Algorithm~\ref{alg:bio}), the model succeeds to whiten synthetic data setup from Section 5.1 when the column vectors of ${\bf V}$ are chosen to be nonnegative.
%      {\bf A)} Error decreases as training progresses. 
%      {\bf B)} Online algorithm performance before and after training.
%      {\bf C)} The learned basis (red) is well-aligned with the generative basis (dashed black) compared to initialization (blue).
%      {\bf D)} Asymmetric feedforward weights, ${\bf W}_{rn}$, and feedback weights, $-{\bf W}_{nr}$, converge to being symmetric.
%     }
%     \label{fig:rebuttal_algo3}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=.5\textwidth]{figures/rebuttal_alpha2.png}
%     \caption{{\bf Impact of $\alpha$ on ${\bf W}_T$ depends on orthogonality of optimal basis.}
%     Using the same synthetic data setup as in Fig.~\ref{fig:synthetic}, we run Algorithm~\ref{alg:online} while varying $\alpha$, with random generative basis, ${\bf V}$, and initial synaptic weight matrix, ${\bf W}_0$, where ${\bf V}$ is either non-orthogonal (blue) orthogonal (orange). Note that the learned basis ${\bf W}_T$ is still considerably improved compared to ${\bf W}_0$ independent of ${\bf V}$ being orthogonal.
%     Means and S.E.M. across 50 random initializations of ${\bf V}$ and ${\bf W}_0$.}
%     \label{fig:rebuttal_alpha}
% \end{figure}
